Personalized PageRank to a Target Node, Revisited

Personalized PageRank (PPR) is a widely used node proximity measure in graph mining and network analysis. Given a source node $s$ and a target node $t$, the PPR value $\pi(s,t)$ represents the probability that a random walk from $s$ terminates at $t$, and thus indicates the bidirectional importance between $s$ and $t$. The majority of the existing work focuses on the single-source queries, which asks for the PPR value of a given source node $s$ and every node $t \in V$. However, the single-source query only reflects the importance of each node $t$ with respect to $s$. In this paper, we consider the {\em single-target PPR query}, which measures the opposite direction of importance for PPR. Given a target node $t$, the single-target PPR query asks for the PPR value of every node $s\in V$ to a given target node $t$. We propose RBS, a novel algorithm that answers approximate single-target queries with optimal computational complexity. We show that RBS improves three concrete applications: heavy hitters PPR query, single-source SimRank computation, and scalable graph neural networks. We conduct experiments to demonstrate that RBS outperforms the state-of-the-art algorithms in terms of both efficiency and precision on real-world benchmark datasets.

==> optimization.tex <==
\section{Optimization}
\vspace{+1mm}

%\hspace*{\fill} \\
%\hspace*{\fill} \\
\vspace{+1mm}
%\subsection{Edge-based $\ell$-hop Backward Push} \label{sec:edgebased_lhoppush}







%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> others.tex <==
\section{Other techniques}
\vspace{+1mm}

%\hspace*{\fill} \\
%\hspace*{\fill} \\




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

